COVID-19: Comparative Analysis of Methods for Identifying Articles Related to Therapeutics and Vaccines without Using Labeled Data

Here we proposed an approach to analyze text classification methods based on the presence or absence of task-specific terms (and their synonyms) in the text. We applied this approach to study six different transfer-learning and unsupervised methods for screening articles relevant to COVID-19 vaccines and therapeutics. The analysis revealed that while a BERT model trained on search-engine results generally performed well, it miss-classified relevant abstracts that did not contain task-specific terms. We used this insight to create a more effective unsupervised ensemble.

==> tex_files/problem_formulation.tex <==
\section{Problem Formulation}
\label{sec:problem}

Our task is to classify the given article into three categories: 1) Vaccine, 2) Therapeutic, and 3) Other, where ``Other" is indicating that given article is neither related to vaccine nor therapeutics. We do this classification based on the relevancy score. Hence, the aim is to generate a relevancy score corresponding to each article. Let $\mathcal{A}= \{a_i\}_{i=1}^n$ denoted a set of $n$ unlabeled research articles. We now formally define our problem as:

\begin{center}
\fbox{\parbox[c]{.9\linewidth}{\textbf{Problem Statement:}
Given a set of unlabeled articles $\mathcal{A}$, learn a generative function, $\mathcal{F} : \mathcal{A} \rightarrow \mathcal{S}$, which can generate relevancy score $s_i \in \mathcal{S}$ for each article $a_i \in \mathcal{A}$.
}}
\end{center}
